Integrated NFV/SDN Architectures: A Systematic Literature Review

Network Functions Virtualization (NFV) and Software-Defined Networking (SDN) are new paradigms in the move towards open software and network hardware. While NFV aims to virtualize network functions and deploy them into general purpose hardware, SDN makes networks programmable by separating the control and data planes. NFV and SDN are complementary technologies capable of providing one network solution. SDN can provide connectivity between Virtual Network Functions (VNFs) in a flexible and automated way, whereas NFV can use SDN as part of a service function chain. There are many studies designing NFV/SDN architectures in different environments. Researchers have been trying to address reliability, performance, and scalability problems using different architectural designs. This Systematic Literature Review (SLR) focuses on integrated NFV/SDN architectures, with the following goals: i) to investigate and provide an in-depth review of the state-of-the-art of NFV/SDN architectures, ii) to synthesize their architectural designs, and iii) to identify areas for further improvements. Broadly, this SLR will encourage researchers to advance the current stage of development (i.e., the state-of-the-practice) of integrated NFV/SDN architectures, and shed some light on future research efforts and the challenges faced.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-siggraph.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-siggraph.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL
